FedLALR: Client-Specific Adaptive Learning Rates Achieve Linear Speedup for Non-IID Data

Federated learning is an emerging distributed machine learning method, enables a large number of clients to train a model without exchanging their local data. The time cost of communication is an essential bottleneck in federated learning, especially for training large-scale deep neural networks. Some communication-efficient federated learning methods, such as FedAvg and FedAdam, share the same learning rate across different clients. But they are not efficient when data is heterogeneous. To maximize the performance of optimization methods, the main challenge is how to adjust the learning rate without hurting the convergence. In this paper, we propose a heterogeneous local variant of AMSGrad, named FedLALR, in which each client adjusts its learning rate based on local historical gradient squares and synchronized learning rates. Theoretical analysis shows that our client-specified auto-tuned learning rate scheduling can converge and achieve linear speedup with respect to the number of clients, which enables promising scalability in federated optimization. We also empirically compare our method with several communication-efficient federated optimization methods. Extensive experimental results on Computer Vision (CV) tasks and Natural Language Processing (NLP) task show the efficacy of our proposed FedLALR method and also coincides with our theoretical findings.

==> 4.5-proof_sketch.tex <==
\section{Proof Sketch of Main results}
In this section, we provide the proof sketch of the Theorem \ref{full-client-theorem}. The detailed proof of Theorem \ref{full-client-theorem}, Theorem \ref{adaptive-interval-theorem}, and above mentioned Remarks are placed in the \textbf{supplementary material} due to limited space.

\begin{proof}[proof sketch]
In this part, we first introduce some notations. In the time window $[tK+1,(t+1)K],$ we denote   $ X_{r,i}:=  x_{t,k,i}$ for   $r=t  K +k$, $1\leq k \leq K$.
Similarly, we define $M_{r,i} = m_{t,k,i}$, $G_{r,i} = g_{t,k,i}$,$V_{r,i}=v_{t,k,i}$,  $\hat{V}_{r,i}=\hat{v}_{t,k,i}$ and  $\theta_{r,i} = \eta_{t,k,i}$.  Using these, we also denote $ \bar{X}_{r} =\frac{1}{N}\sum_{i=1}^{N}X_{r,i}$
 and $(\bar{\theta}_r)_{j} = \frac{1}{\sqrt{\frac{1}{N}\sum_{i=1}^{N}(\hat{V}_{r,i})_{j}}}$.
 
We define  
\begin{align*}
Z_{r} = \bar{X}_{r} + \frac{\beta_{1}}{1 -\beta_{1}}(\bar{X}_{r} - \bar{X}_{r-1}).
\end{align*}
Using the L-smoothness of $f$, we obtain 
\begin{align*}
f(Z_{r+1}) - f(Z_{r}) \leq \langle \nabla f(Z_r),Z_{r+1}-Z_{r} \rangle + \frac{L}{2}\Vert Z_{r+1}-Z_{r} \Vert^2 .
\end{align*}
From lemma 1 we have
\begin{align*}
Z_{r+1}-Z_{r}&= \frac{\alpha \beta_1}{1 - \beta_{1}} \frac{1}{N} \sum_{i} M_{r-1,i} \odot (\theta_{r-1,i} - \theta_{r,i})  -\frac{\alpha \beta_{1}}{1 -\beta_{1}}\frac{1}{N}\sum_{i}\od{( m_{t,k-1,i} -M_{t-1,i}) }{(\theta_{r,i}-\eta_{t,k-1,i})}\nonumber \\
&\qquad - \alpha \frac{1}{N} \sum_{i} G_{r,i} \odot \theta_{r,i}.
\end{align*}

Then we have
\begin{align*}
    f(Z_{r+1}) - f(Z_{r}) 
    & \leq - \alpha \langle \nabla f(Z_r),\frac{1}{N} \sum_{i} G_{r,i} \odot \theta_{r,i} \rangle 
    + \frac{\alpha \beta_1}{1 - \beta_{1}} \langle \nabla f(Z_r),\frac{1}{N} \sum_{i} M_{r-1,i} \odot (\theta_{r-1,i} - \theta_{r,i}) \rangle \nonumber \\
&\quad + \frac{\alpha \beta_1}{1 - \beta_{1}} \ip{\nabla f(Z_{r})}{\frac{1}{N}\sum_{i}\od{( M_{r-1,i} -m_{t,k-1,i})}{(\theta_{r,i}-\eta_{t,k-1,i})}} + \frac{L}{2}\Vert Z_{r+1}-Z_{r} \Vert^2
\end{align*}


Taking expectation on both sides with respect to previous states yields
\begin{align}
&\mathbb{E}_{\xi_r|\xi_{1:r-1}}f(Z_{r+1}) - \mathbb{E}_{\xi_r|\xi_{1:r-1}}f(Z_{r})\leq  \underbrace{- \alpha \mathbb{E}_{\xi_r|\xi_{1:r-1}}\langle \nabla f(Z_r),\frac{1}{N} \sum_{i} G_{r,i} \odot \theta_{r,i} \rangle}_{A1} \nonumber \\
&+ \underbrace{\frac{\alpha \beta_1}{1 - \beta_{1}} \mathbb{E}_{\xi_r|\xi_{1:r-1}}\langle \nabla f(Z_r),\frac{1}{N} \sum_{i} M_{r-1,i} \odot (\theta_{r-1,i} - \theta_{r,i}) \rangle}_{A2} + \underbrace{\frac{L}{2}\mathbb{E}_{\xi_r|\xi_{1:r-1}}\Vert Z_{r+1}-Z_{r} \Vert^2}_{A3}\nonumber \\
&+ \underbrace{\frac{\alpha \beta_1}{1 - \beta_{1}} \EEstr  \langle \nabla f(Z_{r}) , \frac{1}{N}\sum_{i}(M_{r-1,i} - m_{t,k-1,i} )  \odot (\theta_{r,i}-\eta_{t,k-1,i}) \rangle}_{A4} , \label{form:exp}
\end{align}
where the four terms A1,A2,A3,A4 will be calculated in the supplementary materials in detail. We directly present the results here.
 For A1, the first term on RHS of Formula (\ref{form:exp}), is bounded as 
\begin{align*}
&\;\;\;\;- \alpha \mathbb{E}_{\xi_r|\xi_{1:r-1}}\langle \nabla f(Z_r),\frac{1}{N} \sum_{i} G_{r,i} \odot \theta_{r,i} \rangle \leq \frac{\alpha \lambda^2 L^2}{2 \epsilon}\norm{}{Z_{r}-\bar{X}_r} + \frac{\alpha}{2\lambda^2} \norm{}{ \od{ \frac{1}{N} \sum_{i} \nabla f_{i}(X_{r,i})}{\sqrt{\bar{\theta}_{r-1}}}} \nonumber \\
&- \frac{\alpha }{2}\Vert \nabla f(\bar{X}_r) \odot  \sqrt{\bar{\theta}_{r-1}}\Vert^2 - \frac{\alpha }{2} \Vert \frac{1}{N} \sum_{i} \nabla f_{i}(X_{r,i}) \odot  \sqrt{\bar{\theta}_{r-1}} \Vert^2   + \frac{\alpha L^{2}}{2 N \epsilon} \sum_{i} \Vert \bar{X}_r -  X_{r,i}\Vert^2 + \frac{\alpha G_{\infty}^{2}}{2N \epsilon^{3}} \sum_{i} \norm[]{1}{\hat{V}_{r-1,i}-\bar{\hat{V}}_{r-1}}  \nonumber \\
&+ \frac{\alpha G^{2}_{\infty}}{2N \epsilon^3} \EEstr  \sum_{i}  \norm[]{1}{\hat{V}_{r,i}-\hat{V}_{r-1,i}}.
 \end{align*}
Then we bound A2, the second term on RHS of Formula (\ref{form:exp}), in the following formula 
\begin{align*}
&\;\;\;\;\frac{\alpha \beta_1}{1 - \beta_{1}} \EEstr \langle \nabla f(Z_r),\frac{1}{N} \sum_{i} M_{r-1,i} \odot (\theta_{r-1,i} - \theta_{r,i}) \rangle \leq \frac{\alpha \beta_1  G^{2}_{\infty}}{2(1 - \beta_{1})N\epsilon^3} \EEstr \sum_{i} \norm[]{1}{\hat{V}_{r,i} - \hat{V}_{r-1,i}}.
\end{align*}

Next, the third term on RHS of Formula (\ref{form:exp}) A3, is bounded as 
\begin{align*}
&\;\;\;\;\frac{L}{2} \EEstr \Vert Z_{r+1}-Z_{r} \Vert^2 \leq \frac{L}{2} \EEstr  (1+\mu) (\frac{\alpha \beta_1}{1 - \beta_{1}})^2 \frac{G^{2}_{\infty}}{4 \epsilon^{6} N} \sum_{i}\norm{}{\hat{V}_{r,i} - \hat{V}_{r-1,i}} +(1+\frac{1}{\mu})\alpha^2 \frac{L}{2} (\frac{4}{\epsilon} \norm{}{\od{\frac{1}{N} \sum_{i} \nabla f_{i}(X_{r,i})}{\sqrt{\bar{\theta}_{r-1}}}} 
 \nonumber \\
 &+\frac{ G_{\infty}^{2}}{N \epsilon^6}\sum_{i} \norm{}{\hat{V}_{r-1,i}-\bar{\hat{V}}_{r-1}} +  \frac{2d\sigma^2}{N\epsilon^2} + \frac{G^{2}_{\infty}}{2N\epsilon^6}\EEstr (\sum_{i}\norm{}{\hat{V}_{r,i} - \hat{V}_{r-1,i}})).
\end{align*}

Finally,  the fourth term on RHS of Formula (\ref{form:exp}) A4, is bounded as 
\begin{align*}
&\frac{\alpha \beta_1}{1 - \beta_{1}} \EEstr \langle \nabla f(Z_{t}) , \frac{1}{N}\sum_{i} ( M_{r-1,i} -m_{t,k-1,i})\odot (\theta_{r,i}-\eta_{t,k-1,i})\rangle  \leq \frac{\alpha \beta_1}{1 - \beta_{1}} \frac{ G_{\infty}^{2} }{N \epsilon^{3}} \EEstr\sum_{i} \norm[]{1}{\hat{V}_{r,i}-\bar{\hat{V}}_{r-1}}.
\end{align*}

Hence, we  can take  the expectation of the Formula(\ref{form:exp}) and re-arrange it, then we have
\begin{align}
&\;\;\;\;\frac{\alpha}{2}\mathbb{E}\Vert \nabla f(\bar{X}_r) \odot  \sqrt{\bar{\theta}_{r}}\Vert^2 \leq (\mathbb{E}f(Z_{t}) - \mathbb{E}f(Z_{r+1}) ) + \frac{\alpha \lambda^2 L^{2}}{2 \epsilon^{2}}\mathbb{E}\Vert Z_t - \bar{X}_r  \Vert^2 
+ \frac{L^{2} \alpha}{2 N \epsilon^{3}} \mathbb{E}\sum_{i} \Vert \bar{X}_t - X_{r,i}  \Vert^2  + \frac{\alpha G_{\infty}^{2}}{2N \epsilon^{3}} \EE \sum_{i} \norm[]{1}{\hat{V}_{r-1,i}-\bar{\hat{V}}_{r-1}}  \nonumber\\
&\qquad +
 \frac{\alpha G^{2}_{\infty}}{2N \epsilon^2} \EE  \sum_{i}  \norm[]{1}{\hat{V}_{r,i}-\hat{V}_{r-1,i}} + (\frac{\alpha}{2\lambda^2} - \frac{\alpha}{2} +(1+\frac{1}{\mu}) \frac{2L \alpha^2}{\epsilon} )\mathbb{E}\Vert \frac{1}{N} \sum_{i} \nabla f_{i}(X_{r,i}) \odot \sqrt{\bar{\theta}_{r}}  \Vert^2 \nonumber \\
 & +\frac{\alpha \beta_1  G^{2}_{\infty}}{2(1 - \beta_{1})N\epsilon^3} \EE \sum_{i} \norm[]{1}{\hat{V}_{r,i} - \hat{V}_{r-1,i}}+\frac{L}{2} \EE (1+\mu) (\frac{\alpha \beta_1}{1 - \beta_{1}})^2 \frac{G^{2}_{\infty}}{4 \epsilon^{6} N} \sum_{i}\norm{}{\hat{V}_{r,i} - \hat{V}_{r-1,i}} \nonumber \\
&+(1+\frac{1}{\mu})\alpha^2 \frac{L}{2} (\frac{ G_{\infty}^{2}}{N \epsilon^6}\EE \sum_{i} \norm{}{\hat{V}_{r-1,i}-\bar{\hat{V}}_{r-1}} +  \frac{2d\sigma^2}{N\epsilon^2} + \frac{G^{2}_{\infty}}{2N\epsilon^6}\EE \sum_{i}\norm{}{\hat{V}_{r,i} - \hat{V}_{r-1,i}})+ \frac{\alpha \beta_1}{1 - \beta_{1}} \frac{ G_{\infty}^{2} }{N \epsilon^{3}} \EE \sum_{i} \norm[]{1}{\hat{V}_{r,i}-\bar{\hat{V}}_{r-1}}.\label{form:exp7}
\end{align}

 Noticing $\Vert \nabla f(\bar{X}_r) \odot  \sqrt{\bar{\theta}_{r}}\Vert^2 \ge \frac{1}{G_{\infty}}\Vert \nabla f(\bar{X}_r) \Vert^2$, we divide the Formula (\ref{form:exp7}) by $\alpha$ on the both sides and
sum it over $t \in \{0,1,2,...,T-1\}, k \in \{1,2,...,K \}$. And dividing both side of it by $KT$ yields
\begin{align}
&\;\;\;\;\frac{1}{2G_{\infty}}\mathbb{E}[\sum_{r=1}^{KT}\frac{\Vert \nabla f(\bar{X}_r) \Vert^2}{KT}] \leq \underbrace{\frac{\mathbb{E}f(Z_{1}) - \mathbb{E}f(Z_{KT+1})}{\alpha KT}}_{B1} + \underbrace{\frac{ \lambda^2 L^{2}}{2 KT\epsilon^{2}}\mathbb{E}\sum_{r=1}^{KT}\Vert Z_r - \bar{X}_r  \Vert^2}_{B2}  + \underbrace{\frac{L^{2} }{2 N KT\epsilon^{2}} \mathbb{E}\sum_{r=1}^{KT}\sum_{i} \Vert \bar{X}_r - X_{r,i}  \Vert^2}_{B3} \nonumber\\
& + \underbrace{\frac{(2-\beta_1)G_{\infty}^{2}}{2(1-\beta_1)NKT \epsilon^{3}} \EE \sum_{r=1}^{KT}\sum_{i} \norm[]{1}{\hat{V}_{r-1,i}-\bar{\hat{V}}_{r-1}}}_{B4}  +
\underbrace{\frac{ G^{2}_{\infty}}{2NKT \epsilon^3 (1 - \beta_{1})} \EE  \sum_{r=1}^{KT}\sum_{i}  \norm[]{1}{\hat{V}_{r,i}-\hat{V}_{r-1,i}}}_{B5} \nonumber\\ 
& + \underbrace{(\frac{1}{2\lambda^2} - \frac{1}{2} +(1+\frac{1}{\mu}) \frac{2L \alpha}{\epsilon} )\frac{1}{KT}\sum_{r=1}^{KT} \mathbb{E}\Vert \frac{1}{N} \sum_{i} \nabla f_{i}(X_{r,i}) \odot \sqrt{\bar{\theta}_{r}}  \Vert^2}_{B6} + \underbrace{(\frac{L}{2}  (1+\mu) \frac{\alpha \beta_1^2}{(1 - \beta_{1})^2} \frac{G^{2}_{\infty}}{4 \epsilon^{6} NKT} 
+ (1+\frac{1}{\mu})\alpha \frac{L}{2} \frac{G^{2}_{\infty}}{2NKT\epsilon^6})}_{B7}\nonumber \\
&\;\;\;\; \underbrace{\times \EE \sum_{r=1}^{KT}\sum_{i}\norm{}{\hat{V}_{r,i} - \hat{V}_{r-1,i}}}_{B7} +(1+\frac{1}{\mu})\frac{L}{2} (\underbrace{\frac{\alpha  G_{\infty}^{2}}{NKT \epsilon^6}\EE \sum_{r=1}^{KT}\sum_{i} \norm{}{\hat{V}_{r-1,i}-\bar{\hat{V}}_{r-1}}}_{B8} +  \frac{2d\alpha  \sigma^2}{N\epsilon^2} ).\label{form:exp9}
\end{align}


The term B1 of the Formula (\ref{form:exp9}) is bounded as 
\begin{align*}
\frac{\mathbb{E}f(Z_{1}) - \mathbb{E}f(Z_{KT+1})}{\alpha KT} \leq \frac{\mathbb{E}f(Z_{1}) - f^{*}}{\alpha KT} =\frac{f(Z_{1}) - f^{*}}{\alpha KT}.
\end{align*}

The term B2 of the Formula (\ref{form:exp9}) is bounded as
\begin{align*}
&\frac{1}{KT}\mathbb{E}\sum_{r=1}^{KT} \Vert Z_r - \bar{X}_r  \Vert^2 \leq \frac{\alpha^{2}\beta_{1}^{2} G_{\infty}^2 d}{(1 -\beta_{1})^{2} \epsilon^{2}} 
\end{align*}
which follows from Lemma 26.

The term  B3  is bounded as
\begin{align*}
&\frac{1}{NKT} \sum_{r=1}^{KT}\mathbb{E}\sum_{i} \Vert \bar{X}_r - X_{r,i}  \Vert^2 \leq \frac{2K^{2} G_{\infty}^{2}\alpha^{2}}{\epsilon^{2}}(1+ 4K^{2}(1-\beta_{1})^{2} d) 
\end{align*}
which holds due to Lemma 27.

The term B4 is bounded as
\begin{align*}
&\frac{1}{NKT} \EE \sum_{r=1}^{KT}\sum_{i} \norm[]{1}{\hat{V}_{r-1,i}-\bar{\hat{V}}_{r-1}} = \frac{1}{NKT} \EE \sum_{r=1}^{KT-1}\sum_{i} \norm[]{1}{\hat{V}_{r,i}-\bar{\hat{V}}_{r}} \leq \frac{1}{NKT} \EE \sum_{r=1}^{KT}\sum_{i} \norm[]{1}{\hat{V}_{r,i}-\bar{\hat{V}}_{r}} \nonumber\\
&\overset{(a)}{\leq} \frac{2(N-1)Kd(G_{\infty} -\epsilon)}{NKT}\leq \frac{2Kd(G_{\infty}^{2} -\epsilon^{2})}{KT},
\end{align*}
where  (a) follows from Lemma 19.

The  term B5  is bounded as
\begin{align*}
&\frac{ 1}{NKT} \EE  \sum_{r=1}^{KT}\sum_{i}  \norm[]{1}{\hat{V}_{r,i}-\hat{V}_{r-1,i}} \overset{(a)}{\leq} \frac{ (3N-2)d(G_{\infty}^2 - \epsilon^{2}) }{NKT}\leq \frac{ 3d(G_{\infty}^2 - \epsilon^{2}) }{KT},
\end{align*}
where (a) follows from Lemma 20. 

For the term   B6, we choose $\lambda^{2}=4$,$\mu=4$ and $\alpha \leq \frac{3\epsilon}{20L}$,then $(\frac{1}{2\lambda^2} - \frac{1}{2} +(1+\frac{1}{\mu}) \frac{2L \alpha}{\epsilon} )\leq 0$. The term is smaller than 0, so we can throw it away. 

For   B7, we have
\begin{align*}
&\frac{\alpha}{NKT} \EE \sum_{r=1}^{KT}\sum_{i}\norm{}{\hat{V}_{r,i} - \hat{V}_{r-1,i}}\overset{(a)}{\leq} \frac{2\alpha (N-1)d(G_{\infty}^{2}-\epsilon^{2})^{2}}{KT} \leq  \frac{2\alpha Nd(G_{\infty}^{2}-\epsilon^{2})^{2}}{KT},
\end{align*}
where (a) follows from Lemma 25.

For   B8, we have
\begin{align*}
&\frac{\alpha}{NKT} \EE \sum_{r=1}^{KT}\sum_{i}\norm{}{\hat{V}_{r-1,i} - \bar{\hat{V}}_{r-1}} \overset{(a)}{\leq} \frac{ 4K \alpha (N-1)^{2}d^{2}(G_{\infty}^2 - \epsilon^{2})^{2} }{NKT} \leq \frac{ 4K \alpha Nd^{2}(G_{\infty}^2 - \epsilon^{2})^{2} }{KT},
\end{align*}
where (a) follows from Lemma 24.

Choosing $\lambda^{2}=4$, $\mu=4$, the Formula (\ref{form:exp9})    reads
\begin{align}
&\;\;\;\;\frac{1}{2G_{\infty}}\mathbb{E}[\sum_{r=1}^{KT}\frac{\Vert \nabla f(\bar{X}_r) \Vert^2}{KT}] \leq \frac{f(Z_{1}) - f^{*}}{\alpha KT}+ \frac{5L d\sigma^2}{4 \epsilon^2} \frac{ \alpha}{N} + (\frac{2 L^{2} \beta_{1}^{2} G_{\infty}^2 d}{(1 -\beta_{1})^{2} \epsilon^{4}}  +  \frac{K^{2} L^{2} G_{\infty}^{2}}{\epsilon^{4}}(1+ 4K^{2}(1-\beta_{1})^{2} d))\alpha^{2}\nonumber\\
& + (\frac{(2-\beta_1 )G_{\infty}^{2} Kd(G_{\infty}^{2} -\epsilon^{2})}{(1-\beta_1 )\epsilon^{3}} + \frac{3d(G_{\infty}^2 - \epsilon^{2}) G^{2}_{\infty}}{2 \epsilon^3 (1 - \beta_{1})})\frac{1}{KT} +(\frac{5L G^{2}_{\infty} d(G_{\infty}^{2}-\epsilon^{2})^{2}}{8 \epsilon^{6} (1 - \beta_{1})^2}(  2\beta_1^2+(1 - \beta_{1})^2 ) + \frac{5L K G_{\infty}^{2} d^{2}(G_{\infty}^2 - \epsilon^{2})^{2} }{2 \epsilon^6})\frac{\alpha N}{KT}. \label{form:exp92}
\end{align}
Therefore, the proof is  completed. 
\end{proof}




% \subsection{Proof sketch of Theorem \ref{adaptive-interval-theorem}.}
% \begin{proof}[proof sketch]


% The proof procedure is same as previous until we have Formula \ref{form:exp7}. 
% Summing over $t \in \{0,1,2,...,T-1\}, k_{t} \in \{K_{0},K_{1},...,K_{T-1} \}$ and dividing both side by $\sum K_{t}$ yield
% \begin{align}
% &\;\;\;\;\frac{1}{2G_{\infty}}\mathbb{E}[\sum_{r=1}^{\sum K_{t}}\frac{\Vert \nabla f(\bar{X}_r) \Vert^2}{\sum_{t=0}^{T-1} K_{t}}]\nonumber\\
% &\leq \frac{\mathbb{E}f(Z_{1}) - \mathbb{E}f(Z_{KT+1})}{\alpha \sum K_{t}} + \frac{ \lambda^2 L^{2}}{2 \sum K_{t}\epsilon^{2}}\mathbb{E}\sum_{r=1}^{\sum K_{t}}\Vert Z_r - \bar{X}_r  \Vert^2 + \frac{L^{2} }{2 N \sum K_{t}\epsilon^{2}} \mathbb{E}\sum_{r=1}^{\sum K_{t}}\sum_{i} \Vert \bar{X}_r - X_{r,i}  \Vert^2 \nonumber\\
% &\;\;\;\; + \frac{(2-\beta_1 )G_{\infty}^{2}}{2(1-\beta_1 )N \sum K_{t} \epsilon^{3}} \EE \sum_{r=1}^{\sum K_{t}}\sum_{i} \norm[]{1}{\hat{V}_{r-1,i}-\bar{\hat{V}}_{r-1}}  +
%  \frac{ G^{2}_{\infty}}{2N\sum K_{t} \epsilon^3} \EE  \sum_{r=1}^{\sum K_{t}}\sum_{i}  \norm[]{1}{\hat{V}_{r,i}-\hat{V}_{r-1,i}} \nonumber\\ 
%  &\;\;\;\; + (\frac{1}{2\lambda^2} - \frac{1}{2} +(1+\frac{1}{\mu}) \frac{2L \alpha}{\epsilon} )\frac{1}{\sum K_{t}}\sum_{r=1}^{\sum K_{t}} \mathbb{E}\Vert \frac{1}{N} \sum_{i} \nabla f_{i}(X_{r,i}) \odot \sqrt{\bar{\theta}_{r}}  \Vert^2\nonumber\\
%   &\;\;\;\; +\frac{\beta_1  G^{2}_{\infty}}{2(1 - \beta_{1})N\sum K_{t}\epsilon^3} \EE \sum_{r=1}^{\sum K_{t}}\sum_{i} \norm[]{1}{\hat{V}_{r,i} - \hat{V}_{r-1,i}}+\frac{L}{2} (1+\mu) \frac{\alpha \beta_1^2}{(1 - \beta_{1})^2} \frac{G^{2}_{\infty}}{4 \epsilon^{6} N\sum K_{t}} \EE  \sum_{r=1}^{\sum K_{t}}\sum_{i}\norm{}{\hat{V}_{r,i} - \hat{V}_{r-1,i}} \nonumber \\
% &\;\;\;\;+(1+\frac{1}{\mu})\alpha \frac{L}{2} (\frac{ G_{\infty}^{2}}{N\sum K_{t} \epsilon^6}\EE \sum_{r=1}^{\sum K_{t}}\sum_{i} \norm{}{\hat{V}_{r-1,i}-\bar{\hat{V}}_{r-1}} +  \frac{2d\sigma^2}{N\epsilon^2} + \frac{G^{2}_{\infty}}{2N\sum K_{t}\epsilon^6}\EE \sum_{r=1}^{\sum K_{t}}\sum_{i}\norm{}{\hat{V}_{r,i} - \hat{V}_{r-1,i}})\\
% &= \underbrace{\frac{\mathbb{E}f(Z_{1}) - \mathbb{E}f(Z_{1+\sum K_{t}})}{\alpha \sum K_{t}}}_{B1} + \underbrace{\frac{ \lambda^2 L^{2}}{2 \sum K_{t}\epsilon^{2}}\mathbb{E}\sum_{r=1}^{\sum K_{t}}\Vert Z_r - \bar{X}_r  \Vert^2}_{B2} + \underbrace{\frac{L^{2} }{2 N KT\epsilon^{2}} \mathbb{E}\sum_{r=1}^{\sum K_{t}}\sum_{i} \Vert \bar{X}_r - X_{r,i}  \Vert^2}_{B3} \nonumber\\
% &\;\;\;\; + \underbrace{\frac{(2-\beta_1)G_{\infty}^{2}}{2(1-\beta_1)N\sum K_{t} \epsilon^{3}} \EE \sum_{r=1}^{\sum K_{t}}\sum_{i} \norm[]{1}{\hat{V}_{r-1,i}-\bar{\hat{V}}_{r-1}}}_{B4}  +
% \underbrace{\frac{ G^{2}_{\infty}}{2N\sum K_{t} \epsilon^3 (1 - \beta_{1})} \EE  \sum_{r=1}^{\sum K_{t}}\sum_{i}  \norm[]{1}{\hat{V}_{r,i}-\hat{V}_{r-1,i}}}_{B5} \nonumber\\ 
% &\;\;\;\; + \underbrace{(\frac{1}{2\lambda^2} - \frac{1}{2} +(1+\frac{1}{\mu}) \frac{2L \alpha}{\epsilon} )\frac{1}{\sum K_{t}}\sum_{r=1}^{\sum K_{t}} \mathbb{E}\Vert \frac{1}{N} \sum_{i} \nabla f_{i}(X_{r,i}) \odot \sqrt{\bar{\theta}_{r}}  \Vert^2}_{B6}\nonumber\\
% &\;\;\;\; + \underbrace{(\frac{L}{2}  (1+\mu) \frac{\alpha \beta_1^2}{(1 - \beta_{1})^2} \frac{G^{2}_{\infty}}{4 \epsilon^{6} N\sum K_{t}} 
% + (1+\frac{1}{\mu})\alpha \frac{L}{2} \frac{G^{2}_{\infty}}{2N\sum K_{t}\epsilon^6})\EE \sum_{r=1}^{\sum K_{t}}\sum_{i}\norm{}{\hat{V}_{r,i} - \hat{V}_{r-1,i}}}_{B7} \nonumber \\
% &\;\;\;\;+(1+\frac{1}{\mu})\frac{L}{2} (\underbrace{\frac{\alpha  G_{\infty}^{2}}{N\sum K_{t} \epsilon^6}\EE \sum_{r=1}^{\sum K_{t}}\sum_{i} \norm{}{\hat{V}_{r-1,i}-\bar{\hat{V}}_{r-1}}}_{B8} +  \frac{2d\alpha  \sigma^2}{N\epsilon^2} ).
% \end{align}

% In the sequel, let us bound each term on the RHS of the Formula (\ref{form:exp9-adap}).

% The term B1 is bounded as 
% \begin{align}
% \frac{\mathbb{E}f(Z_{1}) - \mathbb{E}f(Z_{1+\sum K_{t}})}{\alpha \sum K_{t}} \leq \frac{\mathbb{E}f(Z_{1}) - f^{*}}{\alpha \sum K_{t}} =\frac{f(Z_{1}) - f^{*}}{\alpha \sum K_{t}}.
% \end{align}

% The term B2 is bounded as
% \begin{align}
% &\frac{1}{\sum K_{t}}\mathbb{E}\sum_{r=1}^{\sum K_{t}} \Vert Z_r - \bar{X}_r  \Vert^2 \leq \frac{\alpha^{2}\beta_{1}^{2} G_{\infty}^2 d}{(1 -\beta_{1})^{2} \epsilon^{2}},
% \end{align}
% which follows from Lemma \ref{lemma:z-xbar-adap}

% The term B3 is bounded as
% \begin{align}
%     &\frac{1}{N\sum K_{t}} \sum_{r=1}^{\sum K_{t}}\mathbb{E}\sum_{i} \Vert \bar{X}_r - X_{r,i}  \Vert^2 \leq \frac{2K^{2}_{T-1} G_{\infty}^{2}\alpha^{2}}{\epsilon^{2}}(1+ 4K^{2}_{T-1}(1-\beta_{1})^{2} d),
% \end{align}
% which follows from Lemma \ref{lemma:xbar-x-adap}

% The term B4 is bounded as
% \begin{align}
% &\frac{1}{N\sum_{\tau=0}^{T-1} K_{\tau}} \EE \sum_{r=1}^{\sum_{\tau=0}^{T-1} K_{\tau}}\sum_{i} \norm[]{1}{\hat{V}_{r-1,i}-\bar{\hat{V}}_{r-1}} = \frac{1}{N\sum_{\tau=0}^{T-1} K_{\tau}} \EE \sum_{r=1}^{\sum_{\tau=0}^{T-1} K_{\tau}-1}\sum_{i} \norm[]{1}{\hat{V}_{r,i}-\bar{\hat{V}}_{r}}  \nonumber\\
% &\leq \frac{1}{N\sum_{\tau=0}^{T-1} K_{\tau}} \EE \sum_{r=1}^{\sum_{\tau=0}^{T-1} K_{\tau}}\sum_{i} \norm[]{1}{\hat{V}_{r,i}-\bar{\hat{V}}_{r}} \overset{(a)}{\leq} \frac{2(N-1)K_{T-1}d(G_{\infty} -\epsilon)}{N\sum_{\tau=0}^{T-1} K_{\tau}}\leq \frac{2K_{T-1}d(G_{\infty}^{2} -\epsilon^{2})}{\sum_{\tau=0}^{T-1} K_{\tau}},
% \end{align}
% where (a) follows from Lemma \ref{lemma:sumt-l1-v-vbar-adap}.

% The term B5 is bounded as
% \begin{align}
% \frac{ 1}{N\sum_{\tau=0}^{T-1} K_{\tau}} \EE  \sum_{r=1}^{\sum_{\tau=0}^{T-1} K_{\tau}}\sum_{i}  \norm[]{1}{\hat{V}_{r,i}-\hat{V}_{r-1,i}} \overset{(a)}{\leq} \frac{ (3N-2)d(G_{\infty}^2 - \epsilon^{2}) }{N\sum_{\tau=0}^{T-1} K_{\tau}} \leq \frac{ 3d(G_{\infty}^2 - \epsilon^{2}) }{\sum_{\tau=0}^{T-1} K_{\tau}},
% \end{align}
% where (a) follows from Lemma \ref{lemma:sumt-l1-v-t-1-adap}. 

% For the term B6 we choose $\lambda^{2}=4$,$\mu=4$, let $\alpha \leq \frac{3\epsilon}{20L}$,then $(\frac{1}{2\lambda^2} - \frac{1}{2} +(1+\frac{1}{\mu}) \frac{2L \alpha}{\epsilon} )\leq 0$. The term is smaller than 0, so we can ignore this term. 

% For the term B7, we have
% \begin{align}
% \frac{\alpha}{N\sum_{\tau=0}^{T-1} K_{\tau}} \EE \sum_{r=1}^{\sum_{\tau=0}^{T-1} K_{\tau}}\sum_{i}\norm{}{\hat{V}_{r,i} - \hat{V}_{r-1,i}}\overset{(a)}{\leq} \frac{2\alpha (N-1)d(G_{\infty}^{2}-\epsilon^{2})^{2}}{\sum_{\tau=0}^{T-1} K_{\tau}}\leq  \frac{2\alpha Nd(G_{\infty}^{2}-\epsilon^{2})^{2}}{\sum_{\tau=0}^{T-1} K_{\tau}},
% \end{align}
% where (a) follows from Lemma \ref{lemma:sumt-l2-square-v-t-1-adap}.

% For the term B8, we have
% \begin{align}
% \frac{\alpha}{N\sum_{\tau=0}^{T-1} K_{\tau}} \EE \sum_{r=1}^{\sum_{\tau=0}^{T-1} K_{\tau}}\sum_{i}\norm{}{\hat{V}_{r-1,i} - \bar{\hat{V}}_{r-1}} \overset{(a)}{\leq} \frac{ 4K_{T-1} \alpha (N-1)^{2}d^{2}(G_{\infty}^2 - \epsilon^{2})^{2} }{N\sum_{\tau=0}^{T-1} K_{\tau}}\leq \frac{ 4K_{T-1} \alpha Nd^{2}(G_{\infty}^2 - \epsilon^{2})^{2} }{\sum_{\tau=0}^{T-1} K_{\tau}},
% \end{align}
% where (a) follows from Lemma \ref{lemma:sumt-l2-square-v-vbar-adap}.

% Choosing $\lambda^{2}=4$,$\mu=4$,the Formula (\ref{form:exp9-adap}) is  changed as 
% \begin{align}
% &\;\;\;\;\frac{1}{2G_{\infty}}\mathbb{E}[\sum_{r=1}^{\sum_{\tau=0}^{T-1} K_{\tau}}\frac{\Vert \nabla f(\bar{X}_r) \Vert^2}{\sum_{\tau=0}^{T-1} K_{\tau}}]\nonumber\\
% &\leq  \frac{f(Z_{1}) - f^{*}}{\alpha \sum_{\tau=0}^{T-1} K_{\tau}} + \frac{ 2 L^{2}}{\epsilon^{2}} \frac{\alpha^{2}\beta_{1}^{2} G_{\infty}^2 d}{(1 -\beta_{1})^{2} \epsilon^{2}} +  \frac{L^{2} }{2\epsilon^{2}}\frac{2K^{2}_{T-1} G_{\infty}^{2}\alpha^{2}}{\epsilon^{2}}(1+ 4K^{2}_{T-1}(1-\beta_{1})^{2} d)\nonumber\\
% & + \frac{(2-\beta_1 )G_{\infty}^{2}}{2(1-\beta_1 ) \epsilon^{3}}\frac{2K_{T-1}d(G_{\infty}^{2} -\epsilon^{2})}{\sum_{\tau=0}^{T-1} K_{\tau}} + \frac{ G^{2}_{\infty}}{2 \epsilon^3 (1 - \beta_{1})}\frac{ 3d(G_{\infty}^2 - \epsilon^{2}) }{\sum_{\tau=0}^{T-1} K_{\tau}}\nonumber\\
% &+\frac{5L G^{2}_{\infty} d(G_{\infty}^{2}-\epsilon^{2})^{2}}{8 \epsilon^{6} (1 - \beta_{1})^2}(  2\beta_1^2+(1 - \beta_{1})^2 )\frac{\alpha N}{\sum_{\tau=0}^{T-1} K_{\tau}} +\frac{5L K_{T-1} G_{\infty}^{2} d^{2}(G_{\infty}^2 - \epsilon^{2})^{2} }{2 \epsilon^6} \frac{  \alpha N }{\sum_{\tau=0}^{T-1} K_{\tau}} + \frac{5L d\sigma^2}{4 \epsilon^2} \frac{ \alpha}{N}\\
% &= \frac{f(Z_{1}) - f^{*}}{\alpha \sum_{\tau=0}^{T-1} K_{\tau}}+ \frac{5L d\sigma^2}{4 \epsilon^2} \frac{ \alpha}{N} + (\frac{2 L^{2} \beta_{1}^{2} G_{\infty}^2 d}{(1 -\beta_{1})^{2} \epsilon^{4}}  +  \frac{K^{2}_{T-1} L^{2} G_{\infty}^{2}}{\epsilon^{4}}(1+ 4K^{2}_{T-1}(1-\beta_{1})^{2} d))\alpha^{2}\nonumber\\
% & + (\frac{(2-\beta_1 )G_{\infty}^{2} K_{T-1}d(G_{\infty}^{2} -\epsilon^{2})}{(1-\beta_1 )\epsilon^{3}} + \frac{3d(G_{\infty}^2 - \epsilon^{2}) G^{2}_{\infty}}{2 \epsilon^3 (1 - \beta_{1})})\frac{1}{\sum_{\tau=0}^{T-1} K_{\tau}}\nonumber\\
% &+(\frac{5L G^{2}_{\infty} d(G_{\infty}^{2}-\epsilon^{2})^{2}}{8 \epsilon^{6} (1 - \beta_{1})^2}(  2\beta_1^2+(1 - \beta_{1})^2 )+ \frac{5L K_{T-1} G_{\infty}^{2} d^{2}(G_{\infty}^2 - \epsilon^{2})^{2} }{2 \epsilon^6})\frac{\alpha N}{\sum_{\tau=0}^{T-1} K_{\tau}}. \label{form:exp92-adap}
% \end{align}

% When taking $\alpha \leq \sqrt{\frac{N}{\sum_{\tau=0}^{T-1} K_{\tau}}}$ into the Formula (\ref{form:exp92-adap}), we obtain 
% \begin{align}
% \mathbb{E}[\sum_{r=1}^{\sum_{\tau=0}^{T-1} K_{\tau}}\frac{\Vert \nabla f(\bar{X}_r) \Vert^2}{\sum_{\tau=0}^{T-1} K_{\tau}}] &\leq C_{1}\frac{1}{\sqrt{N\sum_{\tau=0}^{T-1} K_{\tau}}} +  \frac{N}{\sum_{\tau=0}^{T-1} K_{\tau}}(C_{2,1} +C_{2,2}K_{T-1}^{2} +C_{2,3}K_{T-1}^{4})\\ \nonumber
% &\;\;\;\;+  \frac{1}{\sum_{\tau=0}^{T-1} K_{\tau}}(C_{3,1}K_{T-1} +C_{3,2}) +  (\frac{N}{\sum_{\tau=0}^{T-1} K_{\tau}})^{1.5}(C_{4,1}+C_{4,2}K_{T-1}).
% \label{form:exp93-adap}
% \end{align}
% where $C_{1},C_{2,1},C_{2,2},C_{2,3},C_{3,1},C_{3,2},C_{4,1},C_{4,2}$ are constants, given as
% \begin{align}
% &C_{1} = 2G_{\infty} (f(Z_{1}) - f^{*} + \frac{5L d\sigma^2}{4 \epsilon^2}) \\
% &C_{2,1} = 2G_{\infty} \frac{2 L^{2} \beta_{1}^{2} G_{\infty}^2 d}{(1 -\beta_{1})^{2} \epsilon^{4}}  \\
% &C_{2,2} = 2G_{\infty}  \frac{ L^{2} G_{\infty}^{2}}{\epsilon^{4}}\\
% &C_{2,3} = 2G_{\infty}  \frac{ L^{2} G_{\infty}^{2}}{\epsilon^{4}} 4(1-\beta_{1})^{2} d\\
% &C_{3,1} = 2G_{\infty} \frac{(2-\beta_1 )G_{\infty}^{2} d(G_{\infty}^{2} -\epsilon^{2})}{(1-\beta_1 ) \epsilon^{3}} \\
% &C_{3,2} = 2G_{\infty} \frac{3d(G_{\infty}^2 - \epsilon^{2}) G^{2}_{\infty}}{2 \epsilon^3 (1 - \beta_{1})}\\
% &C_{4,1} = 2G_{\infty} \frac{5L G^{2}_{\infty} d(G_{\infty}^{2}-\epsilon^{2})^{2}}{8 \epsilon^{6} (1 - \beta_{1})^2}(  2\beta_1^2+(1 - \beta_{1})^2 )\\
% &C_{4,2} = 2G_{\infty}  \frac{5L  G_{\infty}^{2} d^{2}(G_{\infty}^2 - \epsilon^{2})^{2} }{2 \epsilon^6}.
% \end{align}

% When we select $K_{t} = O(log(t))$, only the first term of RHS of the Formula \ref{form:exp93-adap} dominates.
% The rest terms decrease faster than the first term when $T$ becomes very large.
% This implies the linear speedup stated in the Theorem 2.




% \end{proof}
